Adaptive Coordination Offsets for Signalized Arterial Intersections using Deep Reinforcement Learning

Coordinating intersections in arterial networks is critical to the performance of urban transportation systems. Deep reinforcement learning (RL) has gained traction in traffic control research along with data-driven approaches for traffic control systems. To date, proposed deep RL-based traffic schemes control phase activation or duration. Yet, such approaches may bypass low volume links for several cycles in order to optimize the network-level traffic flow. Here, we propose a deep RL framework that dynamically adjusts offsets based on traffic states and preserves the planned phase timings and order derived from model-based methods. This framework allows us to improve arterial coordination while maintaining phase order and timing predictability. Using a validated and calibrated traffic model, we trained the policy of a deep RL agent that aims to reduce travel delays in the network. We evaluated the resulting policy by comparing its performance against the phase offsets deployed along a segment of Huntington Drive in the city of Arcadia. The resulting policy dynamically readjusts phase offsets in response to changes in traffic demand. Simulation results show that the proposed deep RL agent outperformed the baseline on average, effectively reducing delay time by 13.21% in the AM Scenario, 2.42% in the Noon scenario, and 6.2% in the PM scenario when offsets are adjusted in 15-minute intervals. Finally, we also show the robustness of our agent to extreme traffic conditions, such as demand surges in off-peak hours and localized traffic incidents

==> Tables/AM_PercentDiff.tex <==
\begin{table}[]
\begin{tabular}{llll}
Interval & Baseline & Deep RL & \% Diff \\
5-min    & 53.1714  & 56.9253 & -7.0600 \\
10-min   & 53.1269  & 55.8653 & -5.1545 \\
15-min   & 53.4576  & 46.3958 & 13.2101 \\
30-min   & 53.1733  & 54.0258 & -1.6032 \\
45-min   & 53.8985  & 54.945  & -1.9416
\end{tabular}
\end{table}

==> Tables/NN_PercentDiff.tex <==
\begin{table}[]
\begin{tabular}{llll}
Interval & Baseline & Deep RL & \% Diff \\
5-min    & 43.1900  & 44.1823 & -2.2975 \\
10-min   & 43.1611  & 44.0133 & -1.9745 \\
15-min   & 43.3667  & 42.3172 & 2.4201  \\
30-min   & 43.2250  & 43.8963 & -1.5530 \\
45-min   & 43.2140  & 43.5669 & -0.8166
\end{tabular}
\end{table}

==> Tables/PM_PercentDiff.tex <==
\begin{table}[]
\begin{tabular}{llll}
Interval & Baseline & Deep RL & \% Diff \\
5-min    & 45.1764  & 47.3423 & -4.7943 \\
10-min   & 45.1562  & 46.5711 & -3.1333 \\
15-min   & 45.8853  & 43.0391 & 6.2029  \\
30-min   & 45.1936  & 46.8821 & -3.7361 \\
45-min   & 45.6022  & 46.5532 & -2.0854
\end{tabular}
\end{table}

==> appendices.tex <==
\appendices

\section*{Schedule of offset configurations}
\begin{table}[ht]
\caption{SYNCHRO Offsets in (a) AM and (b) Noon (c) PM scenarios}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}[width=\columnwidth]{c c c c c c} 
\hline\hline 
\toprule
Time              & Offset 1 & Offset 2 & Offset 3 & Offset 4 & Offset 5 \\ \midrule
5:00 AM - 5:45 AM & 75       & 66       & 14       & 19       & 48       \\ \midrule
5:45 AM - 6:30 AM & 40       & 40       & 5        & 0        & 5        \\ \midrule
6:30 AM - 9:00 AM & 60       & 60       & 65       & 75       & 5        \\ \midrule
9:00AM - 11:00 AM & 40       & 40       & 5        & 0        & 5        \\  \bottomrule
\hline
\hline
\end{tabular}
}
\resizebox{\columnwidth}{!}{%
\begin{tabular}[width=\columnwidth]{c c c c c c} 
\hline\hline 
\toprule
Time                & Offset 1 & Offset 2 & Offset 3 & Offset 4 & Offset 5 \\ \midrule
10:00 AM - 12:00 NN & 40       & 40       & 5        & 0        & 5        \\ \midrule
12:00 NN - 2:00 PM  & 0        & 0        & 55       & 55       & 55       \\ \bottomrule
\hline
\hline
\end{tabular}
}
\resizebox{\columnwidth}{!}{%
\begin{tabular}[width=\columnwidth]{c c c c c c} 
\hline\hline 
\toprule
Time              & Offset 1 & Offset 2 & Offset 3 & Offset 4 & Offset 5 \\ \midrule
2:00 PM - 4:00 PM & 0        & 0        & 55       & 55       & 55       \\ \midrule
4:00 PM - 7:00 PM & 60       & 60       & 65       & 75       & 5        \\ \midrule
7:00 PM - 8:30 PM & 0        & 0        & 55       & 55       & 55       \\ \midrule
8:30 PM - 9:00 PM & 40       & 40       & 5        & 0        & 5        \\ \bottomrule
\hline 
\end{tabular}
}
\label{table:sychoffsets_am} 
\end{table}

\begin{table}[ht]
\caption{Deep RL Offsets in (a) AM and (b) Noon and (c) PM scenarios}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}[width=\columnwidth]{c c c c c c} 
\hline\hline 
\toprule
Time                & Offset 1 & Offset 2 & Offset 3 & Offset 4 & Offset 5 \\ \midrule
5:00 AM - 6:00 AM   & 31       & 8        & 60       & 43       & 6        \\ \midrule
6:00 AM - 8:00 AM   & 31       & 55       & 60       & 43       & 6        \\ \midrule
8:00 AM - 8:15 AM   & 70       & 86       & 82       & 43       & 107      \\ \midrule
8:15 AM - 8:30 AM   & 70       & 86       & 82       & 59       & 107      \\ \midrule
8:30 AM - 8:45 AM   & 37       & 73       & 82       & 59       & 107      \\ \midrule
8:45 AM - 9:15 AM   & 37       & 86       & 82       & 59       & 107      \\ \midrule
9:15 AM - 10:45 AM  & 37       & 73       & 82       & 59       & 107      \\ \midrule
10:45 AM - 11:00 AM & 70       & 86       & 82       & 59       & 107      \\ \bottomrule
\hline
\hline
\end{tabular}
}
\resizebox{\columnwidth}{!}{%
\begin{tabular}[width=\columnwidth]{c c c c c c} 
\hline\hline 
\toprule
Time                & Offset 1 & Offset 2 & Offset 3 & Offset 4 & Offset 5 \\ \midrule
10:00 AM - 11:45 AM & 70       & 86       & 82       & 59       & 107      \\ \midrule
11:45 AM - 12:00 NN & 37       & 72       & 60       & 43       & 107      \\ \midrule
12:00 NN - 12:45 PM & 31       & 55       & 60       & 43       & 6        \\ \midrule
12:45 PM - 1:00 PM  & 31       & 55       & 60       & 71       & 6        \\ \midrule
1:00 PM - 1:15 PM   & 37       & 73       & 82       & 59       & 107      \\ \midrule
1:15 PM - 1:30 PM   & 71       & 72       & 60       & 97       & 48       \\ \midrule
1:30 PM - 1:45 PM   & 71       & 72       & 88       & 97       & 48       \\ \midrule
1:45 PM - 2:00 PM   & 31       & 72       & 60       & 43       & 6        \\ \bottomrule
\hline
\hline
\end{tabular}
}

\resizebox{\columnwidth}{!}{%
\begin{tabular}[width=\columnwidth]{c c c c c c} 
\hline
\hline 
Time              & Offset 1 & Offset 2 & Offset 3 & Offset 4 & Offset 5 \\ \midrule
2:00 PM - 2:30 PM & 50       & 55       & 15       & 43       & 81       \\ \midrule
2:30 PM - 2:45 PM & 71       & 72       & 60       & 43       & 48       \\ \midrule
2:45 PM - 3:00 PM & 31       & 55       & 60       & 43       & 6        \\ \midrule
3:00 PM - 3:30 PM & 71       & 72       & 88       & 97       & 48       \\ \midrule
3:30 PM - 3:45 PM & 31       & 55       & 60       & 43       & 6        \\ \midrule
3:45 PM - 4:15 PM & 71       & 72       & 60       & 97       & 48       \\ \midrule
4:15 PM - 4:30 PM & 31       & 72       & 60       & 43       & 6        \\ \midrule
4:30 PM - 4:45 PM & 31       & 55       & 60       & 97       & 6        \\ \midrule
4:45 PM - 5:15 PM & 31       & 55       & 60       & 43       & 6        \\ \midrule
5:15 PM - 5:30 PM & 71       & 72       & 60       & 97       & 6        \\ \midrule
5:30 PM - 7:45 PM & 31       & 55       & 60       & 43       & 6        \\ \midrule
7:45 PM - 8:00 PM & 71       & 72       & 88       & 97       & 46       \\ \midrule
8:00 PM - 8:45 PM & 31       & 55       & 60       & 43       & 6        \\ \midrule
8:45 PM - 9:00 PM & 19       & 104      & 60       & 72       & 107      \\ \bottomrule
\hline 
\end{tabular}
}
\label{table:sychoffsets_noon_pm} 
\end{table}

==> intro_backup.tex <==
\section{Introduction}
\IEEEPARstart{A}{cross} the world and throughout the years, traffic congestion has been one of the most complex problems that our cities face, especially in the face of our ever-growing economy.
For instance, an average driver in Los Angeles spends up to 11\% of their day stuck in traffic congestion, costing the US economy \$87 billion in 2018~\cite{cookson2017inrix}.
As the demand for transportation increases in urban areas, there is a need to develop systems that help manage traffic congestion.
Arterial roads, in particular, suffer from congestion, and much of the work on optimizing arterial networks are geared towards designing \emph{Intelligent Traffic Signal Control} (ITSC) systems that adapt to the highly dynamic nature of traffic demand~\cite{ezell2010explaining}.
Not only do systems have to adapt to changes rapidly, but also they have to be \emph{coordinated} with neighboring signalized intersections to improve traffic flow. 
Considerable solutions have been proposed to address the traffic signal coordination problem. 
These have led to the development of adaptive control strategies such as MAXBAND~\cite{little1966synchronization}, MULTIBAND~\cite{gartner1991multi}, and TRANSYT~\cite{robertson1969transyt}. 
These passive model-based traffic control systems are typically optimized for a particular demand scenario~\cite{wang2018review}; 
multiple control plans with different phase offsets, which are usually generated by optimization algorithms,
account for the variation of demand throughout the day ~\cite{little1966synchronization, roess2004traffic,zou2004timing}.
A limitation of these algorithms is that they only optimize for particular directions, which can result in congestion, reducing the performance of the whole network and biasing traffic flow for the predefined directions~\cite{gettman2007data}.
Moreover, these systems frame the traffic signal control optimization problem with a static objective function in which certain parameters are just assumed and not learned from actual data.
This affects the robustness of the system against highly-dynamic conditions and exogenous uncertainties (e.g. traffic incidents, demand surges)~\cite{rodrigues2019towards}. 

The advancement of powerful computational capabilities and rising ubiquity of novel data sources has driven new perspectives in solving problems.
In 2015, one of AI's key breakthroughs in the context of control was being able to achieve almost superhuman level as it beat top players in Atari Games~\cite{mnih2015human} and Go~\cite{silver2017mastering} using deep reinforcement learning (RL).
Successfully applying deep RL to transportation has the potential to drastically improve traffic congestion in ways that are difficult to attain using traditional control.


Our proposed approach does not seek to overhaul the current state of practice, but instead to refine the coordination, adaptability, and robustness to changing traffic conditions of these arterial intersections. 
Unlike our proposed model-free deep RL approach, existing methods for traffic control explicitly define cost functions, which makes those method more predictable and reliable in the field. 
Predictability and reliability are difficult to achieve in deep RL because of its high-sensitivity to its hyperparameters~\cite{wu2018variance,wu2017flow}.
However, the goal-oriented aspect of deep RL helps improve the adaptability of existing methods in highly-dynamic conditions.
Hence, we integrate the intervention of deep RL agent that dynamically adjusts phase offsets to reduce travel delays in the network while preserving the phase order and timings obtained through state-of-practice transportation methods such as SYNCHRO.
Our approach rests in the middle ground between existing model-based traffic control methods and model-free deep RL.
The phase splits remain model-based while the coordination is model-free, which to the best of our knowledge, is a first among deep RL control variations.
Apart from that, our work also utilizes an arterial traffic model developed by the Connected Corridors I-210 Pilot~\cite{dion2015connected} that is calibrated and validated by field data~\cite{gan2017estimation,gan2019arterial,bayen2011mobile}.

Our work leverages the potential of deep RL in coordinating a series of signalized intersections along an arterial corridor.
We propose to solve coordination using a deep RL approach.
This results in a policy that is trained to dynamically adjust the phase offsets of a series of signalized intersections and is robust enough to adapt to varying traffic demand scenarios.
% We propose a deep RL approach to coordination and train a policy that dynamically adjusts the phase offsets of a series of signalized intersections, and is robust enough to adapt to varying traffic demand scenarios.
While other works that make use of deep RL have agents that manipulate the signal phases~\cite{Wei2018intellilight, Wei2019presslight, Wei2019colight} or utilize deep RL to solve control systems modeled by non-linear Partial Differential Equations~\cite{belletti2017expert}, we focus on solely on control of the phase offsets, which preserves \emph{fairness} from the perspective of drivers waiting at intersections.
%% NEED A PARAGRAPH EXPLAINING FAIRNESS, cite single intersection control cases before this paragraph.

This article discusses our work on using deep RL to achieve an adaptive coordination of signalized arterial intersections.
In Section \ref{prelim}, we discuss the background of deep RL and the essential parameters of RL formalization.
Section \ref{method} discusses our proposed parameterization of the RL problem, the training configuration, the learning algorithm, and the model in which the training and evaluation operated.
Section \ref{results} provides the results, verifies the algorithm, and evaluates against our baseline.
We also discuss the performance of the policy under specific uncertainties such as demand surge and traffic disturbances.
Lastly, we summarize our results in Section \ref{conclusion}.
